CARTIER: Cartographic lAnguage Reasoning Targeted at Instruction Execution for Robots

This work explores the capacity of large language models (LLMs) to address problems at the intersection of spatial planning and natural language interfaces for navigation. We focus on following complex instructions that are more akin to natural conversation than traditional explicit procedural directives typically seen in robotics. Unlike most prior work where navigation directives are provided as simple imperative commands (e.g., "go to the fridge"), we examine implicit directives obtained through conversational interactions.We leverage the 3D simulator AI2Thor to create household query scenarios at scale, and augment it by adding complex language queries for 40 object types. We demonstrate that a robot using our method CARTIER (Cartographic lAnguage Reasoning Targeted at Instruction Execution for Robots) can parse descriptive language queries up to 42% more reliably than existing LLM-enabled methods by exploiting the ability of LLMs to interpret the user interaction in the context of the objects in the scenario.

==> table.tex <==
\begin{table}[ht]
\begin{center}
% \begin{tabular}{ |p{0.07\linewidth}|p{0.15\linewidth}|p{0.2\linewidth}| p{0.4\linewidth} | }
\begin{tabular}{ |p{0.05\textwidth}|p{0.1\textwidth}|p{0.15\textwidth}| p{0.2\textwidth} | }
\hline
\textbf{Types} & Explicit & Implicit  & Conversational \\ \hline
\textbf{Example} & ``\textit{Get the scissors}'' & ``\textit{I need something to cut this paper with}'' & ``\textit{
Wow, my mom will really  love this card I'm making her for her birthday. 
 It has all of her favorite things  on it -- lilies, rabbits, birds...  I think I'll make it a little smaller than a full page though,  so I guess I'll need something to cut the cardstock with.  Oh, I do hope she likes it!}'' \\ \hline
\textbf{Description} & Solved by noun extraction. & Solved by open-vocabulary models that associate the image embedding of an object to its word embedding. & Solved using large language models that can parse complex and descriptive queries. \\ \hline
\textbf{Methods} & Bixby, Google Assistant, Alexa & VLMaps, CLIP-Fields, CoW, LMNav & CARTIER, NLMap \\
 \hline
\end{tabular}
\end{center}
\centering
\caption{Summary of query types with examples (in black), discussion of minimum technology level required to correctly answer (in dark blue), and examples of methods that use these technologies. \drivkin{this table can probably be compressed in terms of size if we run out of space}}
\label{table:query_types}
\end{table}


